Ensemble-Instruct: Generating Instruction-Tuning Data with a Heterogeneous Mixture of LMs

Using in-context learning (ICL) for data generation, techniques such as Self-Instruct (Wang et al., 2023) or the follow-up Alpaca (Taori et al., 2023) can train strong conversational agents with only a small amount of human supervision. One limitation of these approaches is that they resort to very large language models (around 175B parameters) that are also proprietary and non-public. Here we explore the application of such techniques to language models that are much smaller (around 10B--40B parameters) and have permissive licenses. We find the Self-Instruct approach to be less effective at these sizes and propose new ICL methods that draw on two main ideas: (a) Categorization and simplification of the ICL templates to make prompt learning easier for the LM, and (b) Ensembling over multiple LM outputs to help select high-quality synthetic examples. Our algorithm leverages the 175 Self-Instruct seed tasks and employs separate pipelines for instructions that require an input and instructions that do not. Empirical investigations with different LMs show that: (1) Our proposed method yields higher-quality instruction tuning data than Self-Instruct, (2) It improves performances of both vanilla and instruction-tuned LMs by significant margins, and (3) Smaller instruction-tuned LMs generate more useful outputs than their larger un-tuned counterparts. Our codebase is available at https://github.com/IBM/ensemble-instruct.

==> cross-consistency-constraint.tex <==
\section{Cross Consistency Contraints}

==> figure1_old.tex <==
\begin{figure*}

\begin{tikzpicture}[scale=0.9]
% \fontfamily{qcr}\selectfont

\definecolor{gblue}{rgb}{0.69, 0.88, 0.90}
\definecolor{lgray}{rgb}{0.95, 0.95, 0.95}
\definecolor{lgreen}{rgb}{0.85, 0.98, 0.6}

\def \x {0}
\def \y {0}
\def \hd {90}

\node [draw, double, ultra thick, rounded corners, text width= 3.7cm,fill=black,text=white, minimum height = 50pt,align=center] (seed_tasks) at (\x+50pt,\y+0pt) {175 Human-Annotated Seed Tasks: {\fontfamily{qcr}\selectfont \small \\ instruction, \\input (optional), and output}};
%\node [draw, ultra thick, rounded corners, text width= 3.7cm,fill=lgray,text=black, minimum height = 50pt,align=center] (seed_tasks) at (\x+50pt,\y+0pt) {175 Human-Annotated Seed Tasks: {\fontfamily{qcr}\selectfont \small \\ instruction, \\input (optional), and output}};

\node [draw, rectangle split, rectangle split parts=2,rectangle split part fill={gblue,lgray},rounded corners,text width= 2.4cm,minimum height = 50pt,align=center,  above right = 50pt of seed_tasks.north] (instruct_input)  {Generate new Instructions with Inputs \nodepart{second} \fontfamily{qcr}\selectfont \small 24-shot ICL};
\node [draw, rectangle split, rectangle split parts=2,rectangle split part fill={gblue,lgray},rounded corners,text width= 3cm,minimum height = 50pt,align=center, minimum height = 70 pt, right= \hd * 1.7  pt of instruct_input] (ensemble)  {Consensus Filter\nodepart{second} \fontfamily{qcr}\selectfont \small Exact match for classification and RougeL for generation};
\node [draw,rectangle split, rectangle split parts=2,rectangle split part fill={gblue,lgray},rounded corners,text width= 2.8cm,minimum height = 20pt,align=center,  right = \hd pt of instruct_input.north, anchor = north west] (output1)  {Generate Output\nodepart{second} \fontfamily{qcr}\selectfont \small zero-shot};
\node [draw,rectangle split, rectangle split parts=2,rectangle split part fill={gblue,lgray},rounded corners,text width= 2.8cm,minimum height = 20pt,align=center,  right = \hd pt of instruct_input.south, anchor = south west] (output2)  {Generate Output\nodepart{second} \fontfamily{qcr}\selectfont \small zero-shot};
\node [draw,rectangle split, rectangle split parts=2,rectangle split part fill={gblue,lgray},rounded corners,text width= 2.8cm,minimum height = 20pt,align=center,  below = 20 pt of output2] (output3)  {Generate Output\nodepart{second} \fontfamily{qcr}\selectfont \small 18-shot ICL};

\node [draw, rectangle split, rectangle split parts=2,rectangle split part fill={lgreen,lgray},rounded corners,text width= 2.4cm,minimum height = 50pt,align=center,  below right = 50pt of seed_tasks.south] (input)  {Generate new Instructions  (no Inputs) \nodepart{second} \fontfamily{qcr}\selectfont \small 10-shot ICL};
\node [draw, rectangle split, rectangle split parts=2,rectangle split part fill={lgreen,lgray},rounded corners,text width= 3cm,minimum height = 50pt,align=center, right = \hd * 1.7   pt of input] (ensemble2)  {Consensus Filter\nodepart{second} \fontfamily{qcr}\selectfont \small Exact match for classification and RougeL for generation};
\node [draw,rectangle split, rectangle split parts=2,rectangle split part fill={lgreen,lgray},rounded corners,text width= 2.8cm,minimum height = 20pt,align=center,  right = \hd pt of input.north, anchor = north west] (output1_2)  {Generate Output\nodepart{second} \fontfamily{qcr}\selectfont \small zero-shot};
\node [draw,rectangle split, rectangle split parts=2,rectangle split part fill={lgreen,lgray},rounded corners,text width= 2.8cm,minimum height = 20pt,align=center,  right = \hd pt of input.south, anchor = south west] (output2_2)  {Generate Output\nodepart{second} \fontfamily{qcr}\selectfont \small zero-shot};
\node [draw,rectangle split, rectangle split parts=2,rectangle split part fill={lgreen,lgray},rounded corners,text width= 2.8cm,minimum height = 20pt,align=center,  above = 20 pt of output1_2.north] (output3_2)  {Generate Output\nodepart{second} \fontfamily{qcr}\selectfont \small 15-shot ICL};
\node [draw,double, ultra thick,fill=black,text=white, rounded corners,text width= 2cm,minimum height = 50pt,align=center, right =270pt of seed_tasks] (training)  {Synthetic Training Examples};
%\node [draw,ultra thick,fill=lgray,text=black, rounded corners,text width= 2cm,minimum height = 50pt,align=center, right =270pt of seed_tasks] (training)  {Synthetic Training Examples};

% arrows for top part

\draw [-latex,thick] ([xshift=0.5cm]seed_tasks.north west) to[out=90,in=180] 
node[draw,rounded corners,fill=white,pos=0.6] {LM}
node[below=10pt,right=10pt,pos=0.2,text width= 2cm] {\small tasks with instruction and input}  (instruct_input);
\draw [-latex,thick] ([yshift=-0.6cm]instruct_input.north east) to[out=0,in=180] node[draw,rounded corners,fill=white,pos=0.5] {ILM1} ([yshift=-0.6cm]output1.north west);
\draw [-latex,thick] ([yshift=+0.6cm]instruct_input.south east) to[out=0,in=180] node[draw,rounded corners,midway,fill=white,pos=0.5] {ILM2} ([yshift=+0.6cm]output2.south west);
\draw [-latex,thick] (instruct_input) to[out=270,in=180] node[draw,rounded corners,midway,fill=white,pos=0.5] {LM} (output3);

\draw [-latex,thick] (output1) to[out=0,in=180] ([yshift=-0.58cm]ensemble.north west){};
\draw [-latex,thick] (output2) to[out=0,in=180] ([yshift=+0.58cm]ensemble.south west){};

\draw [-latex,thick] (output3) to[out=0,in=270] ([xshift=+1cm]ensemble.south west){};
\draw [-latex,thick] (ensemble) to[out=0,in=90] ([xshift=+2cm]training.north west){};

% arrows for bottom part

\draw [-latex,thick] ([xshift=0.5cm]seed_tasks.south west) to[out=270,in=180] 
node[draw,rounded corners,fill=white,pos=0.6] {LM}
node[below=10pt,right=10pt,pos=0.2,text width= 2cm] {\small instruction-only tasks}  (input);

\draw [-latex,thick] ([yshift=-0.6cm]input.north east) to[out=0,in=180] node[draw,rounded corners,midway,fill=white,pos=0.5] {ILM1} ([yshift=-0.6cm]output1_2.north west);
\draw [-latex,thick] ([yshift=+0.6cm]input.south east) to[out=0,in=180] node[draw,rounded corners,midway,fill=white,pos=0.5] {ILM2} ([yshift=+0.6cm]output2_2.south west);
\draw [-latex,thick] (input) to[out=90,in=180] node[draw,rounded corners,midway,fill=white,pos=0.5] {LM} (output3_2);

\draw [-latex,thick] (output1_2) to[out=0,in=180] ([yshift=-0.58cm]ensemble2.north west){};
\draw [-latex,thick] (output2_2) to[out=0,in=180] ([yshift=+0.58cm]ensemble2.south west){};

\draw [-latex,thick] (output3_2) to[out=0,in=90] ([xshift=+1cm]ensemble2.north west){};
\draw [-latex,thick] (ensemble2) to[out=0,in=270] ([xshift=+2cm]training.south west){};

\end{tikzpicture}
\caption{High-level overview of Ensemble Instruct algorithm for synthetic instruction data generation -- LM refers to vanilla Language Model and ILM to Instruction tuned Language Models and ICL stands for In Context Learning.}
\label{fig:example_rdf}
\end{figure*}

==> figure1_old2.tex <==


\begin{figure*}

\begin{tikzpicture}[scale=1]
% \fontfamily{qcr}\selectfont

\definecolor{gblue}{rgb}{0.69, 0.88, 0.90}
\definecolor{lgray}{rgb}{0.95, 0.95, 0.95}
\definecolor{lgreen}{rgb}{0.85, 0.98, 0.6}

\def \x {0}
\def \y {0}
\def \hd {110}

% seed tasks
\node [draw, double, ultra thick, rounded corners, text width= 4.5cm,fill=black,text=white, minimum height = 50pt,align=center] (seed_tasks) at (\x+50pt,\y+0pt) {175 Human-Annotated \\Seed Tasks: {\fontfamily{qcr}\selectfont \small \\ instruction, input \\(optional), and output}};

% flow above

\node [draw, rectangle split, rectangle split parts=2,rectangle split part fill={gblue,lgray},rounded corners,text width= 2.8cm,minimum height = 50pt,align=center,  above right = 30pt of seed_tasks.north] (instruct_input)  {Generate synthetic Instructions with Inputs \nodepart{second} \fontfamily{qcr}\selectfont \small use 24 random seed tasks with inputs for ICL};

\node [draw,rectangle split, rectangle split parts=2,rectangle split part fill={gblue,lgray},rounded corners,text width= 2.8cm,minimum height = 20pt,align=center,  right = \hd pt of instruct_input.north, anchor = north west] (output1)  {Generate Output\nodepart{second} \fontfamily{qcr}\selectfont \small no ICL for ILMs};

\node [right = \hd + 20 pt of instruct_input.center,align=center] (top_dots) {\quad  ...  ... ...}; 

\node [draw,rectangle split, rectangle split parts=2,rectangle split part fill={gblue,lgray},rounded corners,text width= 2.8cm,minimum height = 20pt,align=center,  right = \hd pt of instruct_input.south, anchor = south west] (output2)  {Generate Output\nodepart{second} \fontfamily{qcr}\selectfont \small 18 ICL examples};

\draw [decorate,decoration={brace,amplitude=10pt,raise=10pt}](output1.north east) -- (output2.south east) node [black,midway,xshift=0.8cm] (brace1) {};

% flow below
\node [draw, rectangle split, rectangle split parts=2,rectangle split part fill={lgreen,lgray},rounded corners,text width= 2.8cm,minimum height = 50pt,align=center,  below right = 30pt of seed_tasks.south] (input)  {Generate synthetic Instructions  (no Inputs) \nodepart{second} \fontfamily{qcr}\selectfont \small use 10 random instruction only seed tasks for ICL};

\node [draw,rectangle split, rectangle split parts=2,rectangle split part fill={lgreen,lgray},rounded corners,text width= 2.8cm,minimum height = 20pt,align=center,  right = \hd pt of input.north, anchor = north west] (output1_2)  {Generate Output\nodepart{second} \fontfamily{qcr}\selectfont \small no ICL for ILMs};

\node [right = \hd + 20 pt of input.center,align=center] (bottom_dots) {\quad   ...  ... ...}; 

\node [draw,rectangle split, rectangle split parts=2,rectangle split part fill={lgreen,lgray},rounded corners,text width= 2.8cm,minimum height = 20pt,align=center,  right = \hd pt of input.south, anchor = south west] (output2_2)  {Generate Output\nodepart{second} \fontfamily{qcr}\selectfont \small 15 ICL examples};

\draw [decorate,decoration={brace,amplitude=10pt,raise=10pt}](output1_2.north east) -- (output2_2.south east) node [black,midway,xshift=0.8cm] (brace2) {};

% filtered output examples

\node [draw,double, ultra thick,fill=black,text=white, rounded corners,text width= 2cm,minimum height = 50pt,align=center, right =250pt of seed_tasks] (training)  {Synthetic Training Examples};


% arrows for top part

\draw [-latex,thick] ([xshift=0.5cm]seed_tasks.north west) to[out=90,in=180] 
node[draw,rounded corners,fill=white,pos=0.6] {\footnotesize LM/ILM}
node[below=10pt,right=10pt,pos=0.2,text width= 2cm] {\footnotesize tasks with instruction and input}  (instruct_input);

\draw [-latex,thick] ([yshift=-0.6cm]instruct_input.north east) to[out=0,in=180] node[draw,rounded corners,fill=white,pos=0.5] {\footnotesize ILM} ([yshift=-0.6cm]output1.north west);
\draw [-latex,thick] (instruct_input) to[out=0,in=180] node[draw,rounded corners,fill=white,pos=0.5] {\footnotesize LM/ILM} (top_dots);
\draw [-latex,thick] ([yshift=+0.6cm]instruct_input.south east) to[out=0,in=180] node[draw,rounded corners,midway,fill=white,pos=0.5] {\footnotesize LM} ([yshift=+0.6cm]output2.south west);

\draw [-latex,thick] (brace1) to[out=0,in=90]  
node[draw,rectangle split, rectangle split parts=2,rectangle split part fill={gblue,lgray},text width=2.4cm,rounded corners,pos=0.6,align = center] {\small Consensus Filter\nodepart{second} \fontfamily{qcr}\selectfont \small Exact Match or RougeL}
(training);

% arrows for bottom part

\draw [-latex,thick] ([xshift=0.5cm]seed_tasks.south west) to[out=270,in=180] 
node[draw,rounded corners,fill=white,pos=0.6] {\footnotesize LM/ILM}
node[below=10pt,right=10pt,pos=0.2,text width= 2cm] {\small instruction-only tasks}  (input);

\draw [-latex,thick] ([yshift=-0.6cm]input.north east) to[out=0,in=180] node[draw,rounded corners,midway,fill=white,pos=0.5] {\footnotesize ILM} ([yshift=-0.6cm]output1_2.north west);
\draw [-latex,thick] (input) to[out=0,in=180] node[draw,rounded corners,fill=white,pos=0.5] {\footnotesize LM/ILM} (bottom_dots);
\draw [-latex,thick] ([yshift=+0.6cm]input.south east) to[out=0,in=180] node[draw,rounded corners,midway,fill=white,pos=0.5] {\footnotesize LM} ([yshift=+0.6cm]output2_2.south west);

\draw [-latex,thick] (brace2) to[out=0,in=270]  
node[draw,rectangle split, rectangle split parts=2,rectangle split part fill={lgreen,lgray},text width=2.4cm,rounded corners,pos=0.6,align = center] {\small Consensus Filter\nodepart{second} \fontfamily{qcr}\selectfont \small Exact Match or RougeL}
(training);

\end{tikzpicture}
\caption{High-level overview of Ensemble Instruct algorithm for synthetic instruction data generation -- LM refers to vanilla Language Model and ILM to Instruction tuned Language Models and ICL stands for In Context Learning.}
\label{fig:example_rdf}
\end{figure*}

==> statisticstable.tex <==
%\subsection{Statistics}
%\multicolumn{3}{c|}{\textbf{Vanilla Base LM}} & \m
\begin{comment}
\begin{table}
\small
\centering
\begin{tabular}{l|cc|c}
\hline
 & \multicolumn{2}{c|}{\textbf{Instance Type}} & \\
\textbf{Dataset} & \textbf{input-output} & \textbf{output} & \textbf{Total} \\
\hline
\textsc{ei-combo+inst} & 9,100 & 8,943 & 18,043 \\
\textsc{ei-falcon+inst} & 13,526 & 13,000 & 26,526 \\
\hline
\end{tabular}
\caption{Synthetic Data Statistics. \textsc{ei-combo+inst} denotes the combination of \textsc{ei-ul2+inst} and \textsc{ei-neoxt+inst}.}
\label{tab:datastats}
\end{table}
\end{comment}

